Demand-based Scheduling of Mixed-Criticality Sporadic Tasks on One Processor

Strategies that artificially tighten high-criticality task deadlines in low-criticality behaviors have been successfully employed for scheduling mixed-criticality systems. Although efficient scheduling algorithms have been developed for implicit deadline task systems, the same is not true for more general sporadic tasks. In this paper we develop a new demand-based schedulability test for such general mixed-criticality task systems, in which we collectively bound the low- and high-criticality demand of tasks. We show that the new test strictly dominates the only other known demand-based test for such systems. We also propose a new deadline tightening strategy based on this test, and show through simulations that the strategy significantly outperforms all known scheduling algorithms for a variety of sporadic task systems.

==> edfpd.tex <==
\section{EDF-PD: Algorithm, Test, and Dominance}
\label{sec:edfpd}

In this section we first present the Earliest Deadline First - Proportionate Deadlines (EDF-PD) scheduling algorithm and then derive a sufficient schedulability test for it. We also show that EDF-PD is speed-up optimal for implicit deadline dual-criticality sporadic task systems, and prove dominance of the derived schedulability test over the best known test for EDF-VD~\cite{BBA12}.

\subsection{EDF-PD Algorithm}
\label{sec:algorithm}

EDF-PD has a pre-processing phase in which it computes the new artificially constrained deadlines for $HC$ tasks in $\tau$. This phase is described in Algorithm~\ref{alg:preprocessing}. First we compute $x$ using Equation~\eqref{eq:x}. Then we compute the proportionate deadline $PD_i$ for each $HC$ task $\tau_i$ using the assumption that the task is allocated $\frac{(u_i^H-u_i^L)u_i^L}{x}$ of the remaining $LC$ utilization. This is the deadline we will use for scheduling the task when the system is in its $LC$ behavior. For Example~\ref{ex:1} given in Section~\ref{sec:motivation}, the proportionate deadlines are $PD_2 = 19$, $PD_3 = 20*19/37$, and $PD_4 = 20*19/24$.

\begin{algorithm}
\caption{EDF-PD: Pre-processing Phase}
\label{alg:preprocessing} 
\begin{algorithmic}[1]
\vspace{0.1in}
\State Compute $x$ using Equation~\eqref{eq:x} in Section~\ref{sec:motivation}.
\vspace{0.1in}
\State For each $HC$ task $\tau_i$, compute its share of remaining $LC$ utilization as $\frac{(u_i^H-u_i^L)u_i^L}{x}$.
\vspace{0.1in}
\State For each $HC$ task $\tau_i$, compute its proportionate deadline $PD_i$ using the equation $C_{i,L}/PD_i = C_{i,L}/T_i (1 + (u_i^H-u_i^L)/x)$. That is, $PD_i = \frac{xT_i}{x+u_i^H-u_i^L}$.
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:edfpd} presents the EDF-PD run-time scheduling strategy. It uses the Earliest Deadline First (EDF) algorithm to schedule tasks in both $LC$ as well as $HC$ behaviors, on account of the known optimality of EDF for traditional non mixed-criticality task systems~\cite{LiLa73}. While the system is in $LC$ behavior, the deadlines of $HC$ jobs are set based on their proportionate deadlines computed above. When the system switches to $HC$ behavior, all $LC$ jobs are discarded because it is no longer necessary to meet their deadlines. All the $HC$ jobs are then scheduled using their actual deadlines, including those that were active when the switch occurred. That is, for each job of a $HC$ task $\tau_i$, its deadline is set equal to $T_i$ time units from its arrival. It is possible to reset the state of the system back to $LC$ behavior provided no $HC$ job has executed beyond its $LC$ WCET over a certain time interval. Techniques for computing this interval length exist in the literature on mode change protocols~\cite{mode_change_survey04}, and therefore we do not investigate it further here. 

\begin{algorithm}
\caption{EDF-PD: Run-time Scheduling Strategy}
\label{alg:edfpd} 
\begin{algorithmic}[1]
\vspace{0.1in}
\State Let $\Gamma$ denote the current criticality-level of the system. $\Gamma$ is initialized with $LC$.
\vspace{0.1in}
\State Schedule $LC$ and $HC$ tasks in $\tau$ using Earliest Deadline First (EDF) algorithm. In this phase, each job of a $LC$ task $\tau_i$ is given deadline equal to $T_i$ and each job of a $HC$ task $\tau_i$ is given deadline equal to $PD_i$.
\vspace{0.1in}
\State When a $HC$ job executes beyond its $LC$ WCET, the system has entered into $HC$ behavior. Update $\Gamma$ to $HC$, reset the deadline of each $HC$ job to its actual value ($T_i$ time units from its arrival instead of $PD_i$), and remove all $LC$ jobs from the ready queue of the scheduler. Schedule the $HC$ jobs using EDF algorithm.
\vspace{0.1in}
\State For each $HC$ task $\tau_i$, new jobs will be assigned deadlines equal to their actual deadlines, that is $T_i$ time units from arrival. No job of $LC$ task will be scheduled.  
\end{algorithmic}
\end{algorithm}

We now illustrate the functioning of algorithm EDF-PD using Example~\ref{ex:1} presented in Section~\ref{sec:motivation}. 

==> motivating_example.tex <==
\section{Motivating Example}
\label{sec:motivation}

An important concept used by job fixed-priority algorithms EDF-VD~\cite{BBG11} and GREEDY~\cite{EkYi12} is the artificial constraining of $HC$ task deadlines when the system is in its $LC$ behavior. This is possible to do whenever $U_L^L + U_H^L < 1$ for the task system. The benefit of these constrained deadlines is that when the system switches to $HC$ behavior, the $HC$ tasks get additional time to execute before their actual deadlines. Assuming all deadlines are met in the $LC$ behavior, when the switch happens, a $HC$ task has at least "actual deadline - constrained deadline" amount of time before its actual deadline to execute any additional workload. These algorithms of course differ in the mechanism of determining what these constrained deadlines should be for each task. EDF-VD distributes the remaining utilization ($1 - U_L^L - U_H^L$) in proportion to the $LC$ utilization ($u_i^L$) of $HC$ tasks. GREEDY on the other hand, performs a greedy search in the solution space of all possible deadline assignments (it only scans a subset of the entire space). Neither of these approaches however, consider the $HC$ utilization ($u_i^H$) of $HC$ tasks when assigning deadlines. When the switch to $HC$ behavior happens, all the $HC$ tasks must be allocated resources in proportion to their $HC$ utilization. It is then a natural question to ask what happens if we assign deadlines taking $HC$ utilizations into consideration. This is the key idea for the algorithm EDF-PD proposed in this paper, and we now explain it using a simple example.

Consider an implicit deadline dual-criticality sporadic task system comprised of $4$ tasks as shown below.

\begin{example}
\begin{itemize}
\item $\tau_1 = (10, 1, \{ 4, 4\})$
\item $\tau_2 = (20, 2, \{ 2, 3\})$
\item $\tau_3 = (20, 2, \{ 2, 8\})$
\item $\tau_4 = (20, 2, \{ 5, 6\})$
\end{itemize}
\label{ex:1}
\end{example}

It is easy to see that $\max \{ U_L^L + U_H^L, U_H^H \} <= 1$ for this task system. The remaining utilization in $LC$ behavior is $1 - U_L^L - U_H^L = 3/20$. EDF-VD will allocate this utilization in proportion to the $LC$ utilization of tasks. As a result, tasks $\tau_2$ and $\tau_3$ would be allocated the same proportion and task $\tau_4$ will get a higher proportion. If you observe the $HC$ utilization of these tasks, $\tau_3$ has the highest, followed by $\tau_4$ and then $\tau_2$. So in any $HC$ behavior, task $\tau_3$ would have the highest demand, but it is still allocated the lowest proportion of remaining $LC$ utilization by EDF-VD. A similar observation can be made when we compare tasks based on the difference between their $HC$ and $LC$ utilizations. Although task $\tau_3$ has the highest increase in demand when the swtich to $HC$ behavior happens, it does not get the largest proportion of remaining $LC$ utilization under EDF-VD. On the other hand, although tasks $\tau_2$ and $\tau_4$ both have the same increase in demand ($1/20$), $\tau_4$ should receive a larger proportion of remaining $LC$ utilization because it has a larger absolute demand than $\tau_2$. Note that the allocation by EDF-VD is consistent with this latter remark. It can be easily verified that the above task system is not schedulable under EDF-VD based on the schedulability test given in~\cite{BBA12}; $U_H^H + U_H^L*U_L^L/(1-U_L^L) = 17/20 + (9/20)*(8/20)/(12/20) = 17/20 + 6/20 > 1$. 

 The GREEDY algorithm decreases the deadline of $HC$ tasks by one time unit in each iteration until the demand bound function based tests for $LC$ and $HC$ behaviors succeed. If the test for $LC$ behavior fails after a deadline decrease, then the change is reverted back (the algorithm backtracks only one step in this fashion). In each iteration the algorithm chooses a task whose deadline reduction will maximize the decrease in $HC$ demand of the system for a specific time interval (namely the shortest interval for which the tests failed). As a result of this "local" focus on imrpoving the schedulability for the shortest time interval, the algorithm fails to utilize task level properties such as those described in the previous paragraph. It initially reduces the deadlines of all the three $HC$ tasks by one. Then, it alternaltely reduces the deadlines of tasks $\tau_2$ and $\tau_3$ and eventually fails. It fails to recognize that for this task system reducing the deadline of task $\tau_3$ is more beneficial than reducing the deadline of task $\tau_2$ from a "global" schedulability point of view.

We are now ready to present the key idea for algorithm EDF-PD. Consider the following definition of $x$.

\begin{equation}
1 - U_L^L - U_H^L = \frac{1}{x} \sum_{\tau_i \in \mathcal{H}_{\tau}} [(u_i^H - u_i^L) u_i^L]
\label{eq:x}
\end{equation}

Note that $x \geq 0$ because $1 - U_L^L - U_H^L \geq 0$ and $u_i^H - u_i^L \geq 0$ for all $i$. The LHS of Equation~\eqref{eq:x} represents the remaining $LC$ utilization for the task system. Suppose we distribute this remaining utilization in such a manner that each $HC$ task $\tau_i$ is allocated a utilization of $\frac{(u_i^H - u_i^L)u_i^L}{x}$. Observe that in this distribution each task is allocated utilization proportional to its $LC$ utilization ($u_i^L$) as well as to the difference between its $HC$ and $LC$ utilizations ($u_i^H - u_i^L$). In the above example, $x = 19/60$, and therefore the allocation of remaining utilization is $36/380$ to $\tau_3$, $6/380$ to $\tau_2$, and $15/380$ to $\tau_4$. Thus task $\tau_3$ is given the largest share of remaining utilization, followed by task $\tau_4$ and then $\tau_2$. This allocation is consistent with our two earlier observations: $\tau_3$ must get a large proportion of the remaining utilization on account of the big difference between its $HC$ and $LC$ utilizations, and $\tau_4$ must be allocated a larger share when compared to $\tau_2$. In the following section we derive a schedulability test for EDF-PD, which will show that the above task system is schedulable under the algorithm.


